Active recursive Bayesian inference using R\'enyi information measures

Recursive Bayesian inference (RBI) provides optimal Bayesian latent variable estimates in real-time settings with streaming noisy observations. Active RBI attempts to effectively select queries that lead to more informative observations to rapidly reduce uncertainty until a confident decision is made. However, typically the optimality objectives of inference and query mechanisms are not jointly selected. Furthermore, conventional active querying methods stagger due to misleading prior information. Motivated by information theoretic approaches, we propose an active RBI framework with unified inference and query selection steps through Renyi entropy and $\alpha$-divergence. We also propose a new objective based on Renyi entropy and its changes called Momentum that encourages exploration for misleading prior cases. The proposed active RBI framework is applied to the trajectory of the posterior changes in the probability simplex that provides a coordinated active querying and decision making with specified confidence. Under certain assumptions, we analytically demonstrate that the proposed approach outperforms conventional methods such as mutual information by allowing the selections of unlikely events. We present empirical and experimental performance evaluations on two applications: restaurant recommendation and brain-computer interface (BCI) typing systems.

==> text/aziz_additions.tex <==
%\subsection{Approximating Renyi entropy}
%\begin{equation}
%\label{eq:RenyiApprox}
   % \begin{split}
      %  &H_{\alpha}(\sigma \lvert \varepsilon, \Phi, \mathcal{H})\\
       % &= \frac{1}{1-\alpha} E_{\varepsilon \lvert \Phi, \mathcal{H}}\left( \log \sum_\sigma p^\alpha(\sigma\lvert \varepsilon,\phi, \mathcal{H}) \right) \\ 
      %  &= \frac{1}{1-\alpha} E_{\sigma\lvert \mathcal{H}}E_{\varepsilon \lvert \Phi, \mathcal{H}}\left(\log \frac{\sum_\sigma p^\alpha(\varepsilon\lvert \sigma,\phi)p^\alpha(\sigma\lvert\mathcal{H})}{p^\alpha({\varepsilon\lvert\phi,\mathcal{H}})} \right)\\
     %   &= \frac{1}{1-\alpha} E_{\sigma\lvert \mathcal{H}}E_{\varepsilon \lvert \Phi, \mathcal{H}}\left(\log \frac{\sum_\sigma p^\alpha(\varepsilon\lvert \sigma,\phi)p^\alpha(\sigma\lvert\mathcal{H})}
    %    {(\sum_\sigma p(\varepsilon\lvert \sigma,\phi)p(\sigma\lvert\mathcal{H}))^\alpha} \right)\\
     %   &= \frac{1}{1-\alpha} E_{\sigma\lvert \mathcal{H}}E_{\varepsilon \lvert \Phi, \mathcal{H}}\left(\log \frac{\sum_\sigma p^\alpha(\varepsilon\lvert \sigma,\phi)p^\alpha(\sigma\lvert\mathcal{H})}
    %    {(\sum_\sigma p(\varepsilon\lvert \sigma,\phi)p(\sigma\lvert\mathcal{H}))^\alpha} \right)
  %  \end{split}
%\end{equation}
%
%Computing the expectation of the log term is not tractable. For the sake of simplicity, such term can be approximated with uni-modal peaky distribution assumption. This assumption is not realistic but presents a closed-form and working approximation by reducing $p(\varepsilon\lvert \sigma,\phi) \in \lbrace 0,1 \rbrace$. Observe that, in \eqref{eq:RenyiApprox} one can also marginilze over the label definition s.t.;
%\begin{equation}
 %   p(\varepsilon\lvert \sigma,\phi) = \sum_\ell p(\varepsilon\lvert \ell ) p(\ell \varepsilon \sigma, \phi)
%\end{equation}

%\subsection{Limit Case of Renyi}
%Observe that $H_\alpha (\sigma \lvert \varepsilon,\phi,\mathcal{H}) $ is ambiguous where $\alpha =1$. To find the limit, we take the derivative of both numerator and denominator with respect to $\alpha$. 
%\begin{equation*}
 %   \frac{\delta}{\delta \alpha} (1-\alpha) = -1
%\end{equation*}
%\begin{equation*}
 %   \frac{\delta}{\delta \alpha}
%\end{equation*}
\subsection{Proof of Proposition 1}
% policy evaluation
% \begin{prop}
\textbf{Proposition  1.}
    \label{prop:MomentumIsBetter}
    \textit{Given, $p(\ell = 1 \lvert \sigma,\phi)\in \lbrace 0,1 \rbrace$, $\forall (\sigma,\phi)$ for $\alpha \in [0,\infty)$ and $\lambda \geq 0$, given  $a,b\in\mathcal{A}$ and $r,q\in\mathcal{Q}$, where $a$ is the state of the target, $a \neq b$, and $r \neq q$, if $ \ \exists \ \mathcal{H}_{s-1} \ \text{s.t.} \ p(a\lvert\mathcal{H}_{s-1})<p(b\lvert\mathcal{H}_{s-1})$, then}
    \begin{equation*}
        \label{eq:adverserial}
         \begin{array}{ll}
         p\Big(-H_{\alpha}(\sigma| \eps, \phi=q, \mathcal{H}_s) + \lambda M_{\alpha}(\phi=q,\mathcal{H}_s) \\
         \hspace{.5in} > -H_{\alpha}(\sigma| \eps, \phi=r, \mathcal{H}_s) + \lambda M_{\alpha}(\phi=r,\mathcal{H}_s)\Big)\\ [.1in]
        \geq  p \Big(-H_{\alpha}(\sigma| \eps, \phi=q, \mathcal{H}_s)  >  -H_{\alpha}(\sigma| \eps, \phi=r, \mathcal{H}_s) \Big)
        \end{array}
    \end{equation*}
% \end{prop}
%
\begin{proof}
Given $a,b$ as two possible states and $q,r$ as two possible queries such that $p(\ell= 1| \sigma=a,\phi=q) = p(\ell=1 | \sigma=b,\phi=r) = 1$ and $p(\ell= 1| \sigma \neq a,\phi=q) = p(\ell=1 | \sigma \neq b,\phi=r) = 0$. Observe that, according to one to one correspondence in state query tuples; $\sum_\sigma f(\sigma,q) p(\ell|\sigma,q)=f(a,q) + \sum_{\sigma\neq a} f(\sigma,q)$ where $f(\cdot,\cdot)$ represents an arbitrary function with arguments from state space and query space correspondingly. Therefore, objectives for query selection can be represented only by corresponding state variables. For the sake of simplicity we denote:
\begin{itemize}
    \item $H_{\alpha}(q) = H_{\alpha}(\sigma=a| \phi=q ,\mathcal{H}_{s})$, \\ $H_{\alpha}(r) = H_{\alpha}(\sigma=b| \phi=r ,\mathcal{H}_{s})$ 
    \item $M_{\alpha}(q) = M_{\alpha}(\phi=q , \ \mathcal{H}_{s})$, \\ $M_{\alpha}(r) = M_{\alpha}(\phi=r , \mathcal{H}_{s})$
    \item $p(a) = p(a\lvert\mathcal{H}_{s})$, \ $p(b) = p(b\lvert\mathcal{H}_{s})$
    \item $p(a|\varepsilon, q) = p(a|\varepsilon, \phi=q, \mathcal{H}_{s})$, \\ $p(b|\varepsilon, r) = p(b|\varepsilon, \phi=r, \mathcal{H}_{s})$
\end{itemize}
We can define notations for $b$ accordingly and ignore $\lambda$ as it holds $\forall \lambda \geq 0$. 
%
Using the probabilistic identity of sum of random variables, we have:
    \begin{equation*}
    \begin{array}{cc}
     p(A+B>C+D)\geq p(A>C,B>D)= p(A>C\vert B>D ) \\
      p(A>C\vert B>D ) = p(B>D) \ \ \forall A,B,C,D
      \end{array}
    \end{equation*}
Thus we can write;
%
\begin{equation*}
\begin{array}{rl}
    &p\left(-H_{\alpha}(q) + \lambda M_{\alpha}(q) \ > \ -H_{\alpha}(r) + \lambda M_{\alpha}(r) \right) \\
    &\geq p\left(M_{\alpha}(q) > M_{\alpha}(r) |-H_{\alpha}(q)>-H_{\alpha}(r)\right) \times \\  &  \ \ \ p\left(-H_{\alpha}(q)>-H_{\alpha}(r)\ \right)
    \end{array}
\end{equation*}
%
\noindent
Since we are dealing with an adversarial case,  $p(a|\mathcal{H}_{s})<p(b|\mathcal{H}_{s})$. Given condition $-H_\alpha(q)>-H_\alpha(r)$ and $p(a|\mathcal{H}_{s})<p(b|\mathcal{H}_{s})$, for $\alpha > 1$, we have:
%
\begin{equation*}
        \begin{split}
        -H_\alpha(q) &> -H_\alpha(r) 
        \end{split}
    \end{equation*}
%
where $-H_\alpha(\sigma|\mathcal{H}_s) = \displaystyle{\frac{1}{\alpha - 1}}\log{\left(\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\mathcal{H}_s)} \right)}$. Accordingly,
%
\begin{equation*}
        \begin{split}
        \displaystyle{\frac{1}{\alpha-1}}\mathbf{E}\left[\log{\left(\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, q)} \right)}\right] &> \ & \displaystyle{\frac{1}{\alpha-1}}\mathbf{E}\left[\log{\left(\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, r)} \right)}\right] \\[0.2in]
        \displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, q)} &> \displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, r)}
        \end{split}
    \end{equation*}
%
Since for $\alpha > 1$, $p^{\alpha-1}(a) < p^{\alpha-1}(b)$, therefore,
\begin{equation*}
        \begin{split}
        \displaystyle{\frac{\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, q)}}{p^{\alpha-1}(a)}} &> \displaystyle{\frac{\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\eps, r)}}{p^{\alpha-1}(b)}}\\[.1in]
        \displaystyle{\sum_{\sigma \in \mathcal{A}}} \displaystyle{\frac{\ p^{\alpha}(\sigma|\eps, q)}{p^{\alpha-1}(a)}}&> \displaystyle{\sum_{\sigma \in \mathcal{A}}} \displaystyle{\frac{\ p^{\alpha}(\sigma|\eps, r)}{p^{\alpha-1}(b)}}\\[.1in]
        \displaystyle{\frac{1}{\alpha -1}}\log \displaystyle{\sum_{\sigma \in \mathcal{A}}} \displaystyle{\frac{\ p^{\alpha}(\sigma|\eps, q)}{p^{\alpha-1}(a)}}&>  \displaystyle{\frac{1}{\alpha -1}}\log \displaystyle{\sum_{\sigma \in \mathcal{A}}} \displaystyle{\frac{\ p^{\alpha}(\sigma|\eps, r)}{p^{\alpha-1}(b)}}\\
        \end{split}
    \end{equation*}
Since, $p(\ell= 1| \sigma \neq a,\phi=q) = p(\ell=1 | \sigma \neq b,\phi=r) = 0$, according to the definition of $M_{\alpha}$, we can conclude $M_\alpha(q) & > M_\alpha(r)$. Since for $0<\alpha<1$, $p^{\alpha-1}(a) > p^{\alpha-1}(b)$, the same conclusion can be drawn.    

Accordingly, when $p(a) < p(b)$ and $-H_\alpha(q) &> -H_\alpha(r)$, we have $M_\alpha(q) & > M_\alpha(r)$, which means $p\left(M_{\alpha}(q) > M_{\alpha}(r) \ | \ -H_{\alpha}(q)>-H_{\alpha}(r) \right)=1$ for the adversarial case, and
%
\begin{equation*}
\begin{array}{rl}
    &p\left(-H_{\alpha}(q) + \lambda M_{\alpha}(q) \ > \ -H_{\alpha}(r) + \lambda M_{\alpha}(r) \right) \\[.1in]
    &\hspace{.5in}\geq p\left(-H_{\alpha}(q) \ > \ -H_{\alpha}(r)\right)
    \end{array}
\end{equation*}
%
\end{proof}
\noindent
%
\subsection{Proof of Proposition 2}
\textbf{Proposition 2.}
\label{prop:colinearity}
\textit{for $\sigma, \phi \in \mathcal{A}=\{a_1,a_2,\dots,a_{|\mathcal{A}|}\}$, probability points $P(\phi)$, $p_{s}$, and $p_{s-1}$ are collinear, where $p_{s} = (p(a_1|\mathcal{H}_{s}),p(a_2|\mathcal{H}_{s}),\dots,p(a_{|\mathcal{A}|}|\mathcal{H}_{s}))$ and $P(\phi) = (0,0,\dots,1,\dots,0)=\mathbf{1}(\phi=\sigma)$, and $\mathbf{1}$ is an indicator operator.}
%
\begin{proof}
%
Using Bayes' rule, we have,
%
\begin{equation*}
\begin{array}{rl}
\label{eq:bayess1}
    p(\sigma=a_i|\eps, \phi=a_j,\mathcal{H}_{s-1}) &=  p(\sigma|\mathcal{H}_{s-1})\displaystyle{\frac{p(\eps|a_i,a_j)}{p(\eps|a_j)}} \\[.1in]
\end{array}
\end{equation*}
%
\begin{equation*}
\begin{array}{rl}
\label{eq:bayess2}
    p(\sigma=a_i|\eps, \phi=a_j,\mathcal{H}_{s-1})&=p(\sigma|\mathcal{H}_{s-1})\displaystyle{\frac{p(\eps|l=0)}{p(\eps|a_j)}} , \\ & \ \ \forall i,j \in [1,N], i \neq j\\[.1in]
\end{array}
\end{equation*}
%
\begin{equation*}
\begin{array}{rl}
\label{eq:bayess3}
    p(\sigma=a_i|\eps, \phi=a_i,\mathcal{H}_{s-1})&=p(\sigma|\mathcal{H}_{s-1})\displaystyle{\frac{p(\eps|l=1)}{p(\eps|a_i)}}, \\ &  \ \ \forall i \in [1,N] \\[.1in]
\end{array}
\end{equation*}
%
Using the fact that all probability points located in the probability simplex have the property $\sum_{i}p(a_i|\mathcal{H}_s)=1$, 
%
\begin{equation}
\begin{array}{rl}
    k_1=\displaystyle{\frac{p(\eps|l=1)}{p(\eps|\phi=a_j)}}, \ k_2=\displaystyle{\frac{p(\eps|l=0)}{p(\eps|\phi=a_j)}} 
\end{array}
\end{equation}
%
\begin{equation}
\begin{array}{rl}
\label{eq:k1k2}
    k_2=\displaystyle{\frac{1-p(\phi=a_j|\mathcal{H}_{s-1})k_1}{1-p(\phi=a_j|\mathcal{H}_{s-1})}}\\[.1in]
\end{array}
\end{equation}
%
In geometry, any two points $X \in \mathcal{R}^N$ $X_1=(x_{1_1},x_{1_2},\dots,x_{1_N})$, $X_2=(x_{2_1},x_{2_2},\dots,x_{2_N})$ are trivially collinear. The line containing these two points is defined as:
%
\begin{equation}
\begin{split}
    \frac{x_1 - x_{1_1}}{x_{2_1}-x_{1_1}}= \frac{x_2 - x_{1_2}}{x_{2_2}-x_{1_2}} = \dots = \frac{x_N - x_{1_N}}{x_{2_N}-x_{1_N}}
\end{split}
\end{equation}
%
Accordingly, for $|\mathcal{A}|=N$ the line determined by $p_0$ and $p_1$ is defined as:
%
\begin{equation}
\begin{split}
 (l_1): \ \ &\frac{x_1 - p(a_1|\mathcal{H}_{s-1})}{p(a_1|\mathcal{H}_{s})-p(a_1|\mathcal{H}_{s-1})}= \dots= \\
 &\frac{x_j - p(a_j|\mathcal{H}_{s-1})}{p(a_j|\mathcal{H}_{s})-p(a_j|\mathcal{H}_{s-1})}= \dots = \\
 &\frac{x_N - p(a_N,|\mathcal{H}_{s-1})}{p(a_N,|\mathcal{H}_{s})-p(a_N,|\mathcal{H}_{s-1}))}
\end{split}
\end{equation}
%
According to the relationship between $p(a_i|\mathcal{H}_{s-1})$ and $p(a_i|\mathcal{H}_{s})$ in (\ref{eq:bayess2}) and (\ref{eq:bayess3}),
%
\begin{equation}
\begin{split}
 &\frac{x_1 - p(a_1|\mathcal{H}_{s-1})}{p(a_1|\mathcal{H}_{s-1})(k_2-1)}= \dots= \\
 &\frac{x_j - p(a_j|\mathcal{H}_{s-1})}{p(a_j|\mathcal{H}_{s-1})(k_1-1)}= \dots = \\
 &\frac{x_N - p(a_N|\mathcal{H}_{s-1})}{p(a_N|\mathcal{H}_{s-1})(k_2-1)}
\end{split}
\end{equation}
%
If $x=P(\phi=a_j)$ point lies on $(\l_1)$ line, then
%
\begin{equation}
\begin{split}
    &\frac{0 - p(a_1|\mathcal{H}_{s-1})}{p(a_1|\mathcal{H}_{s-1})(k_2-1)}= \dots=\\
    &\frac{1 - p(a_j|\mathcal{H}_{s-1})}{p(a_j|\mathcal{H}_{s-1})(k_1-1)}= \dots = \\
    &\frac{0 - p(a_N|\mathcal{H}_{s-1})}{p(a_N|\mathcal{H}_{s-1})(k_2-1)}
\end{split}
\end{equation}
%
Our proof is completed by showing (\ref{eq:otherJ}) and (\ref{eq:correct}) are correct.
%
\begin{equation}
\label{eq:otherJ}
    \frac{- p(a_i|\mathcal{H}_{s-1})}{p(a_i|\mathcal{H}_{s-1})(k_2-1)}= \frac{1 - p(a_j|\mathcal{H}_{s-1})}{p(a_j|\mathcal{H}_{s-1})(k_1-1)}, \ \ \forall i\in [1,N], \ i\neq j
\end{equation}
%
\begin{equation}
\label{eq:correct}
    \frac{- p(a_i|\mathcal{H}_{s-1})}{p(a_i|\mathcal{H}_{s-1})(k_2-1)}= \frac{- p(a_q|\mathcal{H}_{s-1})}{p(a_q|\mathcal{H}_{s-1})(k_2-1)} \ \ \forall i, q \in [1,N], \ i,q\neq j
\end{equation}
%
Trivially, (\ref{eq:correct}) is correct. Using (\ref{eq:k1k2}), (\ref{eq:otherJ}) is also correct.
%
\begin{equation}
    \frac{- 1}{k_2-1}= \frac{1 - p(a_j|\mathcal{H}_{s-1})}{p(a_j|\mathcal{H}_{s-1})(k_1-1)} \\[.2in]
\end{equation}
%
\begin{equation}
\begin{array}{rl}
    p(a_j|\mathcal{H}_{s-1})(1-k_1)&= (1-p(a_j|\mathcal{H}_{s-1}))(k_2-1) \\[.2in]
    &=  (1 - p(a_j|\mathcal{H}_{s-1}))\left(\displaystyle{\frac{1-p(a_j|\mathcal{H}_{s-1})k_1}{1-p(a_j|\mathcal{H}_{s-1})}} - 1 \right)\\[.2in] 
    &=  (1 - p(a_j|\mathcal{H}_{s-1}))\\
    & \ \left(\displaystyle{\frac{p(a_j|\mathcal{H}_{s-1})-p(a_j|\mathcal{H}_{s-1})k_1}{1-p(a_j|\mathcal{H}_{s-1})}}\right) \\[.2in]
    & = p(a_j|\mathcal{H}_{s-1})(1-k_1)
    \end{array}
\end{equation}
\end{proof}
%
\section{Decision Boundary and Feasible Set in RBI}
\label{sec:Decision Boundary and Feasible Set in RBI}
Stopping criterion in $f_I$ relies on the constraint of the inference step. This constraint forms a feasible set in the simplex and hence determines whether the system should keep querying or make a decision. Applying a pre-defined confidence level $\tau$ over posterior in $f_I$, constructs a decision boundary visualized in Figure~\ref{fig:decsionBoundary} in the probability domain. Therefore, for any sequence $s$, if $p(x) \geq \tau$ at a particular vertex, that vertex is the estimated target. 

Shaded regions in Figure~\ref{fig:decsionBoundary} correspond to feasible set as a function of $\tau$, where $S=\{ p(X) \ \lvert \ p(x^*)\geq\tau \}$. As expected, decreasing $\tau$ enlarges the feasible set in the estimation problem. 

\vspace{.1in}
\noindent
\textbf{How can the decision boundary be changed?}

In the RBI problem, the query objective attempts to select a subset of queries by minimizing the conditional entropy across all directions, where the selected queries should push the posterior toward one of the triangle vertices in Figure~\ref{fig:decsionBoundary}. 

There exists a sequence $s$, where $H_s(X) \leq \tau''$ and $p_s(x)\geq \tau$. To investigate the relationship between $\tau''$ and $\tau$, again we will take advantage of geometrical representation in simplex. Figure~\ref{fig:decsionBoundary} shows $H(X)=\tau''$ and $p(a)=\tau$ boundaries. We can see that, by replacing the posterior constraint in $f_I$ with entropy function, we are in turn enlarging the feasible set, as illustrated in Figure~\ref{fig:decsionBoundary}. It also illustrates that the $H_s(X)$ contour is intersecting with $p(a)=\tau$ at the middle of the line $p(a)=\tau$. the following Lemma shows this fact.
%
\decsionBoundary
%
\begin{lemma}
\label{lemma:simplex}
The decision boundary $p(a)=\tau$ intersects the decision boundary of the entropy $H(X)$ at its maximum, where 
$p(a)=\tau, \ p(x)=\displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}, \ \forall x \in \mathcal{A} \setminus \{a\}$. 
%
\end{lemma}
%
\begin{proof}
%
\begin{equation}
\label{eq:entropyValue}
    \begin{array}{rl}
        H_p(X) &= -p(a)\log{\left(p(a)\right)}-{\displaystyle{\sum_{X \in \mathcal{A} \setminus \{a\}}} p(X)\log{\left(p(X)\right)}} \\[.1in]
        &= -\tau\log{\left(\tau\right)}-{\displaystyle{\sum_{X \in \mathcal{A} \setminus \{a\}}} \displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}\log{\left(\displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}\right)}} \\[.1in]
        &=-\tau\log{\left(\tau\right)}-(1-\tau) \log{\left(\displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}\right)} \\[.1in]
        
        \end{array}
\end{equation}
%
Accordingly, we can conclude that $-\tau\log{\left(\tau\right)}-(1-\tau) \log{\left(\displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}\right)}$ is the maximum of the iso-entropy contour $H(X) \leq \tau''$ in the simplex, where it lies on the $p(a)=\tau$ line as well.
%
\end{proof}
%
Accordingly, for $\tau \geq \displaystyle{\frac{1}{|\matchal{a}|}}$, 
%
\begin{equation}
\label{eq:intersection}
    \begin{array}{rl}
        \tau'' &= -\tau\log{\left(\tau\right)}-(1-\tau) \log{\left(\displaystyle{\frac{1-\tau}{|\mathcal{A}|-1}}\right)} \\[.1in]
        \end{array}
\end{equation}
%
Following \textbf{Lemma}, we denote the intersection point by adopting the notation from;
\begin{equation*}
    v_n(\tau)= [\tau, \displaystyle{\frac{1-\tau}{n-1}},\cdots, \displaystyle{\frac{1-\tau}{n-1}}]
\end{equation*}
Here, $n$ denotes the dimensionality of the categorical state space. Additionally, let us define the following point;
\begin{equation*}
    w_n(\tau)= [\tau, {1-\tau},0,\cdots, 0]
\end{equation*}
Without loss of generality, this point can be generalized to any other side by changing the position of $1-\tau$ with any of the $0$s. By definition of the entropy it is clear that $H_\alpha(v_n(\tau))\geq H_\alpha(w_n(\tau))$ and $H_\infty(v_n(\tau))=H_\infty(w_n(\tau))=\tau$. Therefore, the decision boundary is a linear surface in the simplex. $H_\alpha(v_n(\tau))-H_\alpha(w_n(\tau))$ is correlated the extent of the difference between feasible regions. 
\begin{equation}
    \begin{split}
        H_\alpha(v_n(\tau))-H_\alpha(w_n(\tau)) = \frac{1}{1-\alpha}\log \frac{\tau^\alpha+(n-1)^{1-\alpha}(1-\tau)^{\alpha-1})}{\tau^\alpha + (1-\tau)^\alpha}\\
        \text{specifically for $\alpha=1$:} \ \ H(v_n(\tau))-H(w_n(\tau)) = (1-p)\log(n-1)
    \end{split}
\end{equation}
%
In the following figures we visualize the difference with respect to different $\alpha, n$.
%
 \begin{figure*}[h!]
      \centering
      \subfloat{\includegraphics[width=0.35\textwidth]{supplementary_figs/N=30_dif.pdf}}
        \subfloat{\includegraphics[width=0.35\textwidth]{supplementary_figs/alp=0_dif.pdf}}
        \caption{Difference between entropy values of the probabilities $v_n,w_n$ for a given maximum value $\tau$. Left figure visualizes the difference with differing $\alpha$, right figure visualizes the difference with differing $n$.}
\end{figure*}
It should be noted that for a given $\alpha$, there might be a $\tilde{\tau} \ \text{such that} \ H_{\alpha}(v_n(\tau))=H_{\alpha}(w_n(\tilde{\tau}))$. It is apparent equi-entropy balls can yield completely inside the simplex and hence does not intersect with any of the surfaces. Following figures show the effect of different $\alpha$ values where $n=30$ in (a) and the effect of different $n$ values where $\alpha=1$.
 \begin{figure*}[h!]
      \centering
      \subfloat{\includegraphics[width=0.35\textwidth]{supplementary_figs/N=30_inters.pdf}}
        \subfloat{\includegraphics[width=0.35\textwidth]{supplementary_figs/alp=0_inters.pdf}}
        \caption{Left figure visualizes the corresponding $(\tau,\tilde{\tau})$ tuples where $n=30$ for different $\alpha$ values. Right figure visualizes the corresponding $(\tau,\tilde{\tau})$ tuples where $\alpha=1$ for different alpha $n$ values.}
\end{figure*}
%
It can be observed from both figures equi-entropy balls reside inside the simplex and can force a termination in the estimation not getting closer to one vertex. Therefore $\alpha$ is chosen accordingly with $\tau$ value and the cardinality of the state space in our experiments. E.g. as can be observed if we do not require a high confidence (e.g. $\tau \approx 0.8$) in a populated set (e.g. $n=30$) we avoid using $\alpha << 1$ to avoid dramatic performance loss.






==> text/experiment.tex <==
% Experiment
To assess the SB EEG model, we used a language-model-assisted EEG-based BCI typing system called RSVP Keyboard~\cite{mog15}. This system utilizes RSVP paradigm which stands for Rapid Serial Visual Presentation~\cite{mur14}. In RSVP Keyboard a set of pseudo-randomly ordered symbols are rapidly presented as a time series on a prefixed location on the screen in a pseudo-random order to evoke visual potentials\cite{acq10,orh12}. The system uses a finite set of 28 symbols from the English alphabet, in addition to symbols for space and backspace; that is $\mathcal{D} = \{A, B, C, ..., Z, \_, < \}$.
Each flashing symbol is defined as an EEG \textit{trial}, and a set of trials that have been presented with a small time gap in between (e.g. 200 ms) is called an EEG \textit{sequence}. Each sequence is appended with the top candidate in the alphabet \textit{prospect symbol} as feedback according to the posterior probability after ERP/FRP sequence fusion. This prospect symbol is presented as a single flash as an RSVP trial %with black background and 
in a different color than the regular trials to induce positive or negative FRP in the EEG response depending on the prospect’s correctness. Due to low signal to noise ratio (SNR) of EEG, the system is usually required to query the user with more than one sequence and prospect symbols to achieve a desired confidence level. The set of sequences and prospect symbols which lead to a decision is called an \textit{epoch}. It is assumed that the target symbol remains unchanged at each epoch. Figure~\ref{fig:inference} represents a schematic of EEG sequences in the RSVP Keyboard including a series of
of visual stimuli (alphabet) in an ERP sequence and a feedback stimulus as an FRP sequence. In this example FRP sequence corresponds to a positive response, because it matches with the target symbol at trial 6; the rest of the trials correspond to non-target symbols. \newline
%
\begin{figure}[t!]
\centering
\includegraphics[scale=0.27]{figures/sequence.png}
\caption{\sciptsize{Schematic 
of a sequence for the RSVP Keyboard framework. A series of symbols including non-target and target symbols is shown at a prefixed position on the screen consecutively over time in rapid trial fashion. The sequence starts with a $+$ symbol, which is indicated by the magenta line, the ending of the RSVP sequence, a blank screen, % the blue line does not indicate a blank screen!
is shown with a blue line, and the ending of the sequence, a blank screen, is shown with a purple line. At the end of the sequence, a prospect symbol is appended.}} %The inter-trial interval (ITI) of the RSVP trial is 150 ms, which is shorter than the duration of an ERP and it causes dependency across trials.}}
\label{fig:inference}
\end{figure}
%
The RSVP Keyboard has three important system operation modes that are utilized in this study:\\
{\color{review} (1) \textit{Calibration}: The calibration is used to learn the class-conditional distribution of the ERP (target vs. non-target symbols) and FRP sequences (correct vs. incorrect symbols). A user is asked to focus on a set of predefined target symbols shown on the screen, to record labeled EEG data. 

(2) \textit{Copy Phrase}: This mode is designed to assess the system and the user performance in terms of speed and accuracy in the presence of a language model. The user is given a set of predefined phrases. Each phrase includes a missing word and the user is asked to complete the word.

(3) \textit{Simulation}: This mode is base on a proposed probabilistic simulation framework in \cite{orhan2016probabilistic}. A Copy Phrase task is simulated without user intervention. We use Monte-Carlo sampling to draw samples from class distributions using the class conditional distributions learned from Calibration mode. This mode reports the system performance in terms of speed and accuracy. %the probability of phrase completion, total task duration, and information transfer rate (ITR).

Detailed information about RSVP Keyboard can be found in~\cite{orh12,mog15}.}

==> text/method_old.tex <==
% Method
Conventionally, in the Bayesian framework presented in \eqref{eq:originProb}, $f_I$ is a function of the posterior probability and changes in probability domain and state constraint is a confidence level threshold $\tau$ on the system posterior. Moreover, query selection is typically achieved through information theory-based techniques such as maximizing mutual information (MMI)~\cite{jedynak2012twenty}, which is equivalent to conditional entropy minimization when $\beps_s$ corresponding to the upcoming sequence is not observed. Accordingly, $f_I$ and $f_Q$ objectives are defined as follows. 
%
\begin{equation}
    \label{eq:convMIform}
    \begin{array}{ll}
    (I): &\hat{\sigma} =  \displaystyle{\arg\max_{\sigma}} \  p(\sigma| \mathcal{H}_s) \\[.1in]
    &\text{s.t.} \ p({\sigma}| \mathcal{H}_s) \geq \tau \\[.15in]
    (Q): \  &{\Phi}_{s+1} = \displaystyle{\arg\max_{\Phi}} \ -H(\sigma | \beps_{s}, \Phi, \mathcal{H}_s) 
    \end{array}
\end{equation}
%
Since $-H(\sigma | \beps_{s}, \Phi, \mathcal{H}_s)$ is a submodular and non-increasing set function, the sequential subset query selection can be achieved via a greedy approach by optimizing $f_Q$ for each query with theoretical guarantees~\cite{barron1986entropy,johnson2004fisher,farias2011irrevocable}. Therefore, query selection objective can be reformulated for each query as:
%
\begin{equation}    
    \label{eq:action_value_mmi}
   \begin{array}{ll}
    (Q): \  &\phi^i_{s+1} = \arg\max\limits_{\phi} -H(\sigma| \eps^i_{s+1} , \phi, \mathcal{H}_{s})
   \end{array}
\end{equation}
%
Objectives in \eqref{eq:convMIform} are related to each other through the confidence over estimation. Since feasibility in $(I)$ is defined over posterior probability, and the objective in $(Q)$ addresses the ambiguity, it is difficult to analytically investigate the relationship between these objectives. In this paper we introduce a unified framework that connects the feasibility constraint with query optimization.
%
\subsection{Integrating Inference and Querying Objectives: Using Rényi Information Measures}
\label{sec:Renyi}
The typical objective defined for $f_Q$ in \eqref{eq:convMIform} is based on Shannon entropy. However, the total amount of information measured by Shannon entropy is a measure average of bits of information. There exists alternative measures of information flow, e.g. nonlinear methods, by which we aim to compute the information recursively. We propose to use Rényi information measure~\cite{renyi1961measures,song2001renyi,li2016renyi} to bridge the inference and query problems. Using Rényi information measure, the active RBI formulation can be expressed as the following;
 %There are several general information measures, which are computing the information gained according to a nonlinear function. Here, we used Rényi information measure as a beneficial measure that can integrate the inference and query problems. Using Rényi information measure, the RBI formulation can be expressed as:
%
\begin{equation}
    \label{eq:Renyi_RBI}
    \begin{array}{ll}
    (I): &{\sigma} =  \displaystyle{\arg\max_{\sigma \in \mathcal{A}}} \  p(\sigma| \mathcal{H}_s) \\[.1in]
    &\text{s.t.} \ -H_{\alpha_1}({\sigma}| \mathcal{H}_s) \geq \tau' \\[.15in]
    (Q): \  &{\phi}^{i}_{s+1} = \displaystyle{\arg\max_{\phi \in \mathcal{Q}}} \ -H_{\alpha_2}({\sigma}| \eps^i_{s+1}, \phi, \mathcal{H}_s) \\[.15in]
    \end{array}
\end{equation}
%
where, $\tau'$ is the maximum acceptable ambiguity, $\alpha_1$ and $\alpha_2 \in [0, +\infinity]$. $\alpha$-entropy and conditional entropy are defined as:
%
\begin{equation}
    \label{eq:Renyi_entropy}
    \begin{array}{rl}
         H_{\alpha_{1}}(\sigma|\mathcal{H}_s) = \displaystyle{\frac{1}{1-\alpha_1}}\log{\left(\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\mathcal{H}_s)} \right)}
        \end{array}
\end{equation}
%
\begin{equation}
    \label{eq:Renyi_conentropy}
    \begin{array}{rl}
         H_{\alpha_{2}}(\sigma|\beps, \phi, \mathcal{H}_s) = \displaystyle{\frac{1}{1-\alpha_2}}&\mathbf{E}_{p(\eps|\phi,\mathcal{H}_s)}\\
         &\left[\log{\left(\displaystyle{\sum_{\sigma \in \mathcal{A}} \ p^{\alpha}(\sigma|\beps, \phi, \mathcal{H}_s)} \right)}\right]
        \end{array}
\end{equation}
%
Conclusively, for $\alpha_1=\infinity$ and $\alpha_2=1$ the objectives in (\ref{eq:Renyi_RBI}) and (\ref{eq:convMIform}) are identical. Therefore, $\alpha$ is a tuning hyperparameter that finds a balance between the maximum a posterior condition and Shannon entropy. Moreover, since $-H_{\alpha_2}$ is also a submodular and non-increasing set function, the sequential subset query selection can again be performed via a greedy algorithm. 
%
\subsection{A Posterior Changes-based Objective Function}
\label{sec:An Objective function of Posterior Changes Trajectory}
The proposed framework in (\ref{eq:Renyi_RBI}) is using a measure of expected information gain with the current belief (posterior) of an estimate and results in the N-best selection. However, greedy selections based on posterior might initially suffer if the prior information is misleading, i.e. the adversarial case. To encourage exploration in the query selection, we propose a new objective called \textit{Momentum}, which is a function of posterior changes over sequences. Accordingly, the $f_{Q}$ objective can be expressed as:
%
\begin{equation}
    \label{eq:Renyi_monetum_query}
    \begin{array}{ll}
    (Q): \  &{\phi}^{i}_{s+1} = \displaystyle{\arg\max_{\phi \in \mathcal{Q}}} \ -H_{\alpha_2}({\sigma}| \eps^i_{s+1}, \phi, \mathcal{H}_s) + \lambda M_{\alpha_2}(\phi,\mathcal{H}_s) \\[.15in]
    \end{array}
\end{equation}
%
where 
%
\begin{equation}    
        \label{eq:ave_momentum_query}
        \begin{array}{ll}
        M_{\alpha}(\phi , \mathcal{H}_{s}) &= \displaystyle\frac{1}{s}\displaystyle\sum_{n=0}^{s-1}  m_{\alpha}(\phi , \mathcal{H}_{n}) \\
        & = \displaystyle\frac{1}{s}\displaystyle\sum_{n=0}^{s-1} \displaystyle{\frac{1}{(\alpha - 1)}}\log{\displaystyle{\sum_{\sigma \in \mathcal{A}}}\displaystyle{\frac{p^{\alpha}(\sigma|\mathcal{H}_{n+1})}{p^{{\alpha}-1}(\sigma|\mathcal{H}_{n})}}p(l=1|\sigma,\phi)}
        \end{array}
    \end{equation}
%
Here, $m_{\alpha}(\phi , \mathcal{H}_{n})$ is called \textit{Q-Momentum} and $M_{\alpha_2}(\phi,\mathcal{H}_s)$ is the average Q-Momentum.
%
\SimplexProbTrajectories
%
For given $\Phi$, the Momentum term in the $f_I$ stopping criterion would be only function of the task history as follows.
%
\begin{equation}    
        \label{eq:ave_momentum_stop}
        \begin{array}{ll}
        \mathcal{D}_{\alpha}(\mathcal{H}_{s}) = \displaystyle\frac{1}{s}\displaystyle\sum_{n=0}^{s-1}  d_{\alpha}(\mathcal{H}_{n}) = \displaystyle\frac{1}{s}\displaystyle\sum_{n=0}^{s-1} \displaystyle{\frac{1}{(\alpha - 1)}}\log{\displaystyle{\sum_{\sigma \in \mathcal{A}}}\displaystyle{\frac{p^{\alpha}(\sigma|\mathcal{H}_{n+1})}{p^{{\alpha}-1}(\sigma|\mathcal{H}_{n})}}}
        \end{array}
\end{equation}
%
where $d_{\alpha}(\mathcal{H}_{n})$ is called \textit{I-Momentum} and $\mathcal{D}_{\alpha_2}(\mathcal{H}_s)$ is the average I-Momentum.
%
Accordingly, the unified framework for RBI problem can be expressed as:
%
\begin{equation}
    \label{eq:Renyi_monetum_RBI}
    \begin{array}{ll}
    (I): &{\sigma} =  \displaystyle{\arg\max_{\sigma \in \mathcal{A}}} \  p(\sigma| \mathcal{H}_s) \\[.1in]
    &\text{s.t.} \ -H_{\alpha_1}({\sigma}| \mathcal{H}_s) + \lambda_1 \mathcal{D}_{\alpha_1}(\mathcal{H}_s)\geq \tau' \\[.15in]
    (Q): \  &{\phi}^{i}_{s+1} = \displaystyle{\arg\max_{\phi \in \mathcal{Q}}} \ -H_{\alpha_2}({\sigma}| \eps^i_{s+1}, \phi, \mathcal{H}_s) + \lambda_2 M_{\alpha_2}(\phi,\mathcal{H}_s) \\[.15in]
    \end{array}
\end{equation}
%
The pseudocode of the approach is shown in Algorithm~\ref{alg:Active Inference for Decision Making}.
% algorithm
\begin{algorithm}[!t]
\label{alg:proposed_greedy}
\caption{Greedy approach for solving the active recursive Bayesian inference}
\label{alg:Active Inference for Decision Making}
\begin{algorithmic}[1]
\State \textbf{initialize} $\mathcal{A}, \mathcal{Q},\alpha_1\in[0,\infty) , \alpha_2\in[0,\infty), \tau'$
\State $s\gets 0,\mathcal{H_s}\gets \lbrace \mathcal{H}_0 \rbrace$
\While{ $\text{stop} > \tau'$}
\State $\mathcal{Q}'\gets \mathcal{Q}$
\For{ $i \in [0,I]$} \Comment{Batch query selection}
    \State ${\phi}^{i}_{s+1} \gets {\arg\max_{\phi \in \mathcal{Q}'}} \ -H_{\alpha_2}({\sigma}| \eps^i_{s+1}, \phi, \mathcal{H}_s) + \lambda_2 M_{\alpha_2}(\phi,\mathcal{H}_s)$ \Comment{\eqref{eq:Renyi_monetum_RBI}}
    \State $\mathcal{Q}' \gets \mathcal{Q}' \setminus \lbrace {\phi}^{i}_{s+1}\rbrace$
\EndFor
\State $\varepsilon_{s+1} \sim \text{dist-user}(\Phi_{s+1},\sigma)$ \Comment{Observe evidence}
\State $\mathcal{H}_{s+1} \gets \mathcal{H}_{s} \cup \lbrace \varepsilon_{s+1}, \phi_{s+1} \rbrace$ \Comment{Update History}
\State $s\gets s+1$
\State $\text{stop}\gets -H_{\alpha_1}({\sigma}| \mathcal{H}_s) + \lambda_1 \matchal{D}_{\alpha_1}(\mathcal{H}_s)$ \Comment{\eqref{eq:Renyi_monetum_RBI}}
\EndWhile
\State $\hat{{\sigma}} =  \displaystyle{\arg\max_{\sigma \in \mathcal{A}}} \ p(\sigma| \mathcal{H}_s)$
\State \textbf{return} $\hat{\sigma}$
\end{algorithmic}
\end{algorithm}
%
\subsection{Analytical Evaluation} 
\label{subsec:Analytical Evaluation}
For the same given task history, the proposed $f_Q$ in (\ref{eq:Renyi_monetum_RBI}) has higher probability to select the target state compared to the $f_Q$ objective in (\ref{eq:Renyi_RBI}) for adversarial cases.
\newline
%
\begin{prop}
    \label{prop:MomentumIsBetter}
    Given, $p(\ell = 1 \lvert \sigma,\phi)\in \lbrace 0,1 \rbrace$, $\forall (\sigma,\phi)$ for $\alpha \in [0,\infty)$ and $\lambda \geq 0$, given  $a,b\in\mathcal{A}$ and $r,q\in\mathcal{Q}$, where $a$ is the state of the target, $a \neq b$, and $r \neq q$, if $ \ \exists \ \mathcal{H}_{s-1} \ \text{s.t.} \ p(a\lvert\mathcal{H}_{s-1})<p(b\lvert\mathcal{H}_{s-1})$, then
    \begin{equation*}
        \label{eq:adverserial}
        \begin{split}
         &p\left(-H_{\alpha}(\sigma| \eps, \phi=q, \mathcal{H}_s) + \lambda M_{\alpha}(\phi=q,\mathcal{H}_s) \ > \\ &-H_{\alpha}(\sigma| \eps, \phi=r, \mathcal{H}_s) + \lambda M_{\alpha}(\phi=r,\mathcal{H}_s)\right)\\ 
        &\hspace{1cm} \geq \ p\left(-H_{\alpha}(\sigma| \eps, \phi=q, \mathcal{H}_s) \ > \ -H_{\alpha}(\sigma| \eps, \phi=r, \mathcal{H}_s)\right)
        \end{split}
    \end{equation*}
\end{prop}
%
Proposition~\ref{prop:MomentumIsBetter} shows that the probability of $a$ (assumed to be the target state) having a higher $f_Q$ value than $b$ is larger when (\ref{eq:Renyi_monetum_query}) is used instead of $f_Q$ in (\ref{eq:Renyi_RBI}). Although, the probability of $a$ given the task history is lower than the probability of $b$ given the task history. This means that even if $a$ is less likely than $b$ according to the prior (adversarial case) and observed evidence, using the proposed query selection objective, $a$ has more chance to appear in the query subset, when compared to using \eqref{eq:action_value_mmi}.  

It should be noted that, by collecting more evidences trough the recursive process, $\lambda_2$ should be updated dynamically such that the emphasis on $H_{\alpha_2}$ is increased with the number of sequences (\textit{asymptotic convergence}); i.e., the $\lambda$ value should be decreased as the number of sequences is increasing~\cite{bilmes2000dynamic}.
%
\subsection{Geometrical Representation for RBI Problem}
\label{sec:Geometrical Representation for RBI Problem}
To offer better understanding of the proposed unified active RBI framework, in this section, a geometrical view using \textit{probability simplex} is discussed. An important advantage of such a geometrical representation is that it allows us to consider the estimation problem as a posterior trajectory movement tracking, in which we gain new probabilistic insights on the decision boundary, direction and speed of the movement toward a particular state during an active inference. 

Probability mass functions can be visualized geometrically as points in a vector space called a probability simplex with the axis given by random variables. Figure~\ref{fig:simplex_trajectory} illustrates an example of a probability simplex, where each vertex corresponds to a state where its single probability value is set to 1. For simplicity, here we visualize all the findings for fixed cardinality $|\mathcal{A}|$=3. Stopping criterion in $f_I$ relies on the constraint of the inference step. This constraint forms a feasible set in the simplex and hence determines whether the system should keep querying or make a decision. Applying a pre-defined confidence level $\tau$ over posterior in $f_I$, constructs a decision boundary in the probability domain. Therefore, for any sequence $s$, if $p(x) \geq \tau$ at a particular vertex, that vertex is the estimated target.  
%
\subsubsection{Posterior Trajectory Movement}
\label{sec:Posterior Trajectory Movement}
As discussed before, for a single query $\phi$ asked in the RBI framework, the posterior probability is updated according to the \textit{Bayes rule}, which implies that at each sequence, the posterior change is equivalent to $p(\sigma | \mathcal{H}_{s-1})\left[\displaystyle{\frac{p(\eps|\sigma, \phi)}{p(\beps|\phi)}}- 1\right]$. Accordingly, the direction of the posterior change is a function of $\displaystyle{\frac{p(\eps|\sigma, \phi)}{p(\eps|\phi)}}$, called \textit{likelihood evidence ratio}. In fact, query selection directly influences the direction of the posterior trajectory movement in the simplex domain. Figure~
\ref{fig:simplex_trajectory} illustrates an example of posterior movement trajectory moving toward vertex $a$ in the simplex over multiple sequences in the simplex at three stages, (a) beginning of the process, where the system query states \textit{c} and \textit{b} according to the latest probability, however negative responses have been received for both cases; (b) the system proceeds the querying by asking \textit{c} and \textit{b} up to $s=4$, where the system asked \textit{a} and received a corresponding positive response; and (c) where system only queried \textit{a}. Accordingly, there are two questions that can be asked for the posterior trajectory: 1) Can we eliminate the repeated missteps toward non-target vertices? 2) Is it possible to predict the next location of $p_s$ in the simplex and stop earlier?

\textbf{How does Momentum improve the query selection?} 
For the presented posterior trajectory in Figure~\ref{fig:simplex_trajectory}, it was discussed that query selection directly influences the direction of the posterior trajectory movement in the simplex. Using Bayesian method, the direction of the posterior change is a function of $\displaystyle{\frac{p(\eps|\sigma, \phi)}{p(\eps|\phi)}}$. 
%
\begin{prop}
\label{prop:colinearity}
for $\sigma, \phi \in \mathcal{A}=\{a_1,a_2,\dots,a_{|\mathcal{A}|}\}$, probability points $P(\phi)$, $p_{s}$, and $p_{s-1}$ are collinear, where $p_{s} = (p(a_1|\mathcal{H}_{s}),p(a_2|\mathcal{H}_{s}),\dots,p(a_{|\mathcal{A}|}|\mathcal{H}_{s}))$ and $P(\phi) = (0,0,\dots,1,\dots,0)=\mathbf{1}(\phi=\sigma)$, and $\mathbf{1}$ is an indicator operator.
\end{prop}
%
According to Proposition~\ref{prop:colinearity}, prior, posterior and the vertex point corresponding to the query are collinear (proof can be found in the supplementary material). The objective of $f_Q$ should be increasing the chance of guiding the posterior toward $a$. For the adversarial case (Figure~\ref{fig:simplex_proterior}), $H_{\alpha}$ cannot make a correct decision about the the movement direction. However, the proposed Q-Momentum increases the chance of moving toward the target vertex by considering the history of changes rather than latest posterior.
%

\textbf{How can we speed up the estimation process?} Figures~\ref{fig:simplex_probChanges} and \ref{fig:simplex_stopping} show two different querying scenarios where $p(a)<1$. Although for neither case the probability reaches 100\% confidence level, in \ref{fig:simplex_stopping} it is fairly close to the vertex \textit{a}. Therefore, spending an extra query only to reach a pre-defined confidence is not wise. The proposed I-Momentum objective as stopping rule of $f_I$, provides a prediction about the next position of $p_{s+1}$ in the simplex, in which the system can make a decision before passing the decision boundary, which accelerates the inference process. Detailed discussion can be found in the supplementary material. 

